AugGPT: Leveraging ChatGPT for Text Data Augmentation

Text data augmentation is an effective strategy for overcoming the challenge of limited sample sizes in many natural language processing (NLP) tasks. This challenge is especially prominent in the few-shot learning scenario, where the data in the target domain is generally much scarcer and of lowered quality. A natural and widely-used strategy to mitigate such challenges is to perform data augmentation to better capture the data invariance and increase the sample size. However, current text data augmentation methods either can't ensure the correct labeling of the generated data (lacking faithfulness) or can't ensure sufficient diversity in the generated data (lacking compactness), or both. Inspired by the recent success of large language models, especially the development of ChatGPT, which demonstrated improved language comprehension abilities, in this work, we propose a text data augmentation approach based on ChatGPT (named AugGPT). AugGPT rephrases each sentence in the training samples into multiple conceptually similar but semantically different samples. The augmented samples can then be used in downstream model training. Experiment results on few-shot learning text classification tasks show the superior performance of the proposed AugGPT approach over state-of-the-art text data augmentation methods in terms of testing accuracy and distribution of the augmented samples.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> draft.tex <==


%Textual classification is the key problem in Nature language processing.However, it is hard for us to train the NLP model since the limited amount of training data in some scenarios.For limited training dataset, few-shot learning are proposed and become a super popular research field. But the performance doesnot meet the expectation due to the low quality of training dataset.To overcome this challenge, data augmentation has become an increasingly popular technique for improving the generalization capabilities of machine learning models. For previous data augmentation, they do increase the size of training dataset but might not preserve the label or disturb the true label space in the training dataset. Inspired by current popular large language model for its ability to rephrase sentence without changing the semantic meaning, which is the requirement as data augmentation.Thus, we propose a novel approach for few-shot learning with data augmentation by using ChatGPT.Unlike traditional data augmentation, we rephrase each sentence into several samples with the same label. And feed these augmented data for training.  Our results show that using ChatGPT as a data augmentation tool can effectively enrich the training dataset and lead to state-of-the-art performance on taxonomy tasks. This work contributes to the development of new techniques for improving the performance of machine learning models in scenarios with limited data.




%sentence 1: big pic
Textual classification is the key problem in Nature language processing.
%sentence 2: scanario: limited data
However, it is hard for us to train the NLP model since the limited amount of training data in some scenarios.
%sentence 3: few shot leanring may resolve this problem, but performance is not good.
For limited training dataset, few-shot learning are proposed and become a super popular research field. But the performance doesnot meet the expectation due to the low quality of training dataset.

%sentence 4: alternatively, data augmentation
To overcome this challenge, data augmentation has become an increasingly popular technique for improving the generalization capabilities of machine learning models. 
%sentence 5: the problem of previous data augmentation
For previous data augmentation, they do increase the size of training dataset but might not preserve the label or disturb the true label space in the training dataset. 

%=================== why LLM/ChatGPT?
Inspired by current popular large language model for its ability to rephrase sentence without changing the semantic meaning, which is the requirement as data augmentation.

%sentence 6: inspired/motivated by, we ....
Thus, we propose a novel approach for few-shot learning with data augmentation by using ChatGPT.
%sentence 7-8: how?
Unlike traditional data augmentation, we rephrase each sentence into several samples with the same label. And feed these augmented data for training.  
%sentence 9: results
Our results show that using ChatGPT as a data augmentation tool can effectively enrich the training dataset and lead to state-of-the-art performance on taxonomy tasks. 
%sentence 9: summary
This work contributes to the development of new techniques for improving the performance of machine learning models in scenarios with limited data.

The task of few-shot learning for taxonomy is made difficult by the scarcity of labeled training data. To tackle this issue, data augmentation has become a prevalent method for enhancing the generalization of machine learning models. Our research presents a new approach for data augmentation by leveraging ChatGPT, resulting in the preservation of label quality during sentence rephrasing. Our findings demonstrate that incorporating ChatGPT as a data augmentation technique effectively expands the training dataset and attains state-of-the-art results in taxonomy tasks. This contribution advances the advancement of new strategies for enhancing the performance of machine learning models in situations with limited data.

% introduct few data augmentation works here. Then introduce large langauge model.  Language model achieve a state-of-the-art performance in many tasks. 

1. few-shot learning for taxonomy problem 
2. The importance of data augmentation 
3. Why Large language model is helpful?
4. We are the first one who consider the large language model as data augmentation tool.

5. Crucially, our work represents the first method to combine large language models and data augmentation for few-shot learning in taxonomy task.





\begin{table}[t]
\centering
\caption{ Data Augmentation Ablation Study on Symptoms }
\label{table3}
{
\begin{tabular}{ll}
\hline
methods                                      & Sim.  \\
ContextualWordAugUsingBert(Insert)           & 0.954 \\
ContextualWordAugUsingBert(Substitute)       & 0.946 \\
ContextualWordAugUsingDistilBERT(Insert)     & 0.953 \\
ContextualWordAugUsingDistilBERT(Substitute) & 0.943 \\
ContextualWordAugUsingRoBERTA(Insert)        & 0.953 \\
ContextualWordAugUsingRoBERTA(Substitute)    & 0.949 \\
CounterFittedEmbeddingAug                    & 0.953 \\
DeleteCharAugmentation                       & 0.938 \\
DeleteWordAug                                & 0.938 \\
InsertCharAugmentation                       & 0.936 \\
InsertWordByGoogleNewsEmbeddings             & 0.947 \\
KeyboardAugmentation                         & 0.936 \\
OCRAugmentation                              & 0.947 \\
PPDBSynonymAug                               & 0.948 \\
SpellingAugmentation                         & 0.944 \\
SubstituteCharAugmentation                   & 0.935 \\
SubstituteWordByGoogleNewsEmbeddings         & 0.941 \\
SwapCharAugmentation                         & 0.940 \\
SwapWordAug                                  & 0.943 \\
WordNetSynonymAug                            & 0.946 \\
ChatAug                                      & \textbf{0.955} \\
 \hline
\end{tabular}
}
\end{table}


\begin{table}[t]
\centering
\caption{ Data Augmentation Ablation Study on PubMed20K }
\label{table4}
{
\begin{tabular}{ll}
\hline
methods                                      & Sim. \\
ContextualWordAugUsingBert(Insert)           & 0.953           \\
ContextualWordAugUsingBert(Substitute)       & 0.950           \\
ContextualWordAugUsingDistilBERT(Insert)     & 0.951           \\
ContextualWordAugUsingDistilBERT(Substitute) & 0.949           \\
ContextualWordAugUsingRoBERTA(Insert)        & 0.950           \\
ContextualWordAugUsingRoBERTA(Substitute)    & 0.948           \\
CounterFittedEmbeddingAug                    & 0.953           \\
DeleteCharAugmentation                       & 0.947           \\
DeleteWordAug                                & 0.939           \\
InsertCharAugmentation                       & 0.946           \\
InsertWordByGoogleNewsEmbeddings             & 0.948           \\
KeyboardAugmentation                         & 0.946           \\
OCRAugmentation                              & 0.952           \\
PPDBSynonymAug                               & 0.951           \\
SpellingAugmentation                         & 0.945           \\
SubstituteCharAugmentation                   & 0.946           \\
SubstituteWordByGoogleNewsEmbeddings         & 0.945           \\
SwapCharAugmentation                         & 0.948           \\
SwapWordAug                                  & 0.944           \\
WordNetSynonymAug                            & 0.950           \\
ChatAug                                     & \textbf{0.961}  \\
 \hline
\end{tabular}
}
\end{table}



\begin{table}[t]
\centering
\caption{ Data Augmentation Ablation Study on Symptoms }
\label{table5}
{
\begin{tabular}{ll}
\hline
methods                                      & Transrate \\
ContextualWordAugUsingBert(Insert)           & 74.526    \\
ContextualWordAugUsingBert(Substitute)       & 82.450    \\
ContextualWordAugUsingDistilBERT(Insert)     & 75.316    \\
ContextualWordAugUsingDistilBERT(Substitute) & 81.968    \\
ContextualWordAugUsingRoBERTA(Insert)        & 72.186    \\
ContextualWordAugUsingRoBERTA(Substitute)    & 80.175    \\
CounterFittedEmbeddingAug                    & 59.769    \\
DeleteCharAugmentation                       & 71.897    \\
DeleteWordAug                                & 74.484    \\
InsertCharAugmentation                       & 73.543    \\
InsertWordByGoogleNewsEmbeddings             & 74.724    \\
KeyboardAugmentation                         & 74.904    \\
OCRAugmentation                              & 64.016    \\
PPDBSynonymAug                               & 75.005    \\
SpellingAugmentation                         & 74.778    \\
SubstituteCharAugmentation                   & 75.119    \\
SubstituteWordByGoogleNewsEmbeddings         & 79.235    \\
SwapCharAugmentation                         & 70.742    \\
SwapWordAug                                  & 65.830    \\
WordNetSynonymAug                            & 73.787    \\
ChatAug                                     & \textbf{86.718}   \\
 \hline
\end{tabular}
}
\end{table}



\begin{table}[t]
\centering
\caption{ Data Augmentation Ablation Study on PubMed20K }
\label{table6}
{
\begin{tabular}{ll}
\hline
methods                                      & Transrate \\
ContextualWordAugUsingBert(Insert)           & 35.122    \\
ContextualWordAugUsingBert(Substitute)       & 38.604    \\
ContextualWordAugUsingDistilBERT(Insert)     & 35.128    \\
ContextualWordAugUsingDistilBERT(Substitute) & 38.967    \\
ContextualWordAugUsingRoBERTA(Insert)        & 36.094    \\
ContextualWordAugUsingRoBERTA(Substitute)    & \textbf{39.044}    \\
CounterFittedEmbeddingAug                    & 28.006    \\
DeleteCharAugmentation                       & 36.724    \\
DeleteWordAug                                & 34.242    \\
InsertCharAugmentation                       & 36.246    \\
InsertWordByGoogleNewsEmbeddings             & 35.917    \\
KeyboardAugmentation                         & 36.680    \\
OCRAugmentation                              & 33.365    \\
PPDBSynonymAug                               & 32.412    \\
SpellingAugmentation                         & 35.791    \\
SubstituteCharAugmentation                   & 36.818    \\
SubstituteWordByGoogleNewsEmbeddings         & 37.953    \\
SwapCharAugmentation                         & 35.136    \\
SwapWordAug                                  & 33.465    \\
WordNetSynonymAug                            & 35.333    \\
ChatAug                                     & 38.613    \\
 \hline
\end{tabular}
}
\end{table}
